Semantics for a Turing-complete Reversible Programming Language with Inductive Types

This paper is concerned with the expressivity and denotational semantics of a functional higher-order reversible programming language based on Theseus. In this language, pattern-matching is used to ensure the reversibility of functions. We show how one can encode any Reversible Turing Machine in said language. We then build a sound and adequate categorical semantics based on join inverse categories, with additional structures to capture pattern-matching. We then derive a full completeness result, stating that any computable, partial injective function is the image of a term in the language.

==> garbageremoval.tex <==

\subsection{A Canonical Representation}

We define a canonical representation of closed values of some type $A$ into a new
type $\opn{Enc} = \mathbb{B} \oplus \one \oplus \one \oplus \one \oplus \one \oplus \natT$
(recall that $\mathbb{B} = \one\oplus \one$ and $\natT = \mu X. \one\oplus X$).
%
For simplicity let us name each the following terms of type $\opn{Enc}$ : 
\[
	\begin{array}{c}
		\ttt = \inl{(\inl{()})}, \  
		\fff = \inl{(\inr{()})}, \ 
		S = \inr{(\inl{()})}, \ 
		D^\oplus = \inr{(\inr{(\inl{()})})}, \\
		D^\otimes = \inr{(\inr{(\inr{(\inl{()})})})}, \quad 
		D^\mu = \inr{(\inr{(\inr{(\inr{(\inl{()})})})})}, 
	\end{array}
\]
%
and for every natural number $n$, we write $\tilde{n}$ for 
$\inr{(\inr{(\inr{(\inr{(\inr{(\inr{(\overline{n})})})})})})}$.
%
Now, given some closed type $A$, we can define $\floor{-}_A : A\iso
[\opn{Enc}]$ the iso that transform any close value of type $A$ into a list of
$\opn{Enc}$. The iso is defined inductively over $A$.

\begin{definition}[Canonical Encoding]\rm
  $\floor{-}_A$ is defined inductively on $A$ by
  \(\floor{-}_\one = \{() \iso [S]\}\),
  \[\floor{-}_{A\oplus B} = \left\{\begin{array}{lcl}
    \inl{(x)} & \iso & \letv{y}{\floor{x}_A}{D^\oplus :: \fff :: y} \\
    \inr{(x)} & \iso & \letv{y}{\floor{x}_B}{D^\oplus :: \ttt :: y} 
  \end{array}\right\},\]
  \[\floor{-}_{A \otimes B} = \left\{\begin{array}{lcl}
    \pv{x}{y} & \iso & \letv{x'}{\floor{x}_A}{}
                       \letv{y'}{\floor{y}_B}{} \\
              & & \letv{\pv{z}{n}}{++~\pv{x'}{y'}}{} 
                  D^\otimes :: \tilde{n} :: z 
  \end{array}\right\},\]
  \[\floor{-}_{\mu X. A} = \left\{\begin{array}{lcl}
    \fold{x} & \iso & \letv{y}{\floor{x}_{A[X \leftarrow \mu X. A]}}{} 
    D^\mu :: y
  \end{array}\right\},\]
where the iso $++ : [A]\otimes [A] \iso [A]\otimes \natT$ is defined as:
\[\fix f. \left\{\begin{array}{lcl}
  \pv{[]}{x} & \iso & \pv{x}{0} \\
  \pv{h :: t}{x} & \iso & \letv{\pv{y}{n}}{f~\pv{t}{x}}{}
  \pv{h :: y}{S(n)}
\end{array}\right\}.\]
\end{definition}


% \begin{lemma}[$\floor{-}_A$ is well-defined only on closed values]
% 	If $v : A$ is not a close value then $\floor{v} : A$ end up in a stuck state,
% 	i.e. a term of the form $\omega~v'$ for some $\omega$ and $v'$. Conversely,
% 	if $v : A$ is a closed value then $\floor{v} : A$ reduces to a closed value
% 	of type $[\opn{Enc}]$.\qed
% \end{lemma}
% \begin{proof}
%   If $v$ is not closed then one of its subterm is a variable $x$, and for all
%   type $A$, not iso $\floor{x}_A$ matches, hence the term will become stuck when
%   reaching the subterm $x$.
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%       GARBAGE HANDLING    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Getting rid of the garbage}
As we mentioned, often in order to realise some operation in a reversible way,
one need to add some additional garbage. Nevertheless, there exists a way to
remove this garbage, albeit at the cost of a heavier computation time. First
described in~\cite{bennett1973logical}, given two Turing machines $f_1$ and
$f_2$ and some input $\opn{in}$ such that if $f_1(\opn{in}) = \opn{out} \otimes
\opn{garbage}$ and $f_2(\opn{out}) = \opn{in} \otimes \opn{garbage'}$, then the
process consist of taking additional tapes in the Turing Machine in order to
reversibly duplicate (represented by the $\oplus$) or reversibly erase some data
(represented by the $\chi$) in order to recover only the output of $f_1$,
without any garbage. The process is shown in~\Cref{fig:garbage-removal}.

\begin{figure}
  \tikzfig{no-to-garbage}
  \caption{Reversibly removing additional garbage from some process.}
  \label{fig:garbage-removal}
\end{figure}

In order to recreate this process, one therefore need a reversible duplication
process and a reversible erasure process. The two process are obviously the
inverse from one another and so we only focus on the duplication one.
%
Note that every closed value of a closed type can be reversibly duplicated. 


\begin{definition}[Duplication]\rm
  We define $\dup_A^S$ the iso of type $A\iso A\otimes A$ which can duplicate
  any close value of type $A$ by induction on $A$, where $S$ is a set of pairs
  of a type-variable $X$ and an iso-variable $\isovar$, such that for every
  free-variable $X \subseteq A$, there exists a pair $(X, \isovar) \in S$ for
  some $\isovar$.
  %
  The iso is defined by induction on $A$: $\dup_\one^S = \{() \iso \pv{()}{()}\}$, and

  \begin{itemize}
    \item $\dup_{A\otimes B}^S = \left\{\begin{array}{lcl}
      \pv{x}{y} & \iso & \letv{\pv{x_1}{x_2}}{\dup_A^S~x}{} 
       \letv{\pv{y_1}{y_2}}{\dup_B^S~y}{} \\
			&& \pv{\pv{x_1}{y_1}}{\pv{x_2}{y_2}}
    \end{array}\right\}$;
% 
    \item $\dup_{A\oplus B}^S = \left\{\begin{array}{lcl}
      \inl{(x)} & \iso & \letv{\pv{x_1}{x_2}}{\dup_A^S~x}{} 
      \pv{\inl{(x_1)}}{\inl{(x_2)}} \\[0.5em]
      \inr{(y)} & \iso & \letv{\pv{y_1}{y_2}}{\dup_B^S~y}{} 
      \pv{\inr{(y_1)}}{\inr{(y_2)}}
    \end{array}\right\}$;
%
    \item $\dup_{\mu X. A}^S = \left\{\begin{array}{lcl}
				\set{\fix\isovar. \set{\fold{(x)} & \iso &
			\letv{\pv{x_1}{x_2}}{Dup_{A[X\leftarrow\mu X. A]}^{S'}~x}{} \\
			&& \pv{\fold{(x_1)}}{\fold{(x_2)}}}}
    \end{array}\right\}$
    
    if $(X, \_) \not\in S$ and where $S' = S\cup \set{(X , \isovar)}$;

    \item $\dup_{\mu X. A}^S = \set{x \iso \letv{\pv{x_1}{x_2}}{\isovar~x}{\pv{x_1}{x_2}}}$
    where $(X, \isovar) \in S$.
  \end{itemize}
\end{definition}

\begin{lemma}[Properties of Duplication]
  \label{lem:duplication-invariant}
  \label{lem:duplication-typed}
  Given a closed type $A$, then $\dup_A^\emptyset$ is well-defined,
  and the iso $\dup_A^\emptyset$ is well typed of type
  $A\iso A\otimes A$.\qed
\end{lemma}

\begin{lemma}[Semantics of Duplication]
  \label{lem:duplication-semantics}
  Given a closed type $A$ and a closed value $v$ of type $A$, then
  $\dup_A^\emptyset~v \to^* \pv{v_1}{v_2}$ and $v = v_1 = v_2$;
	and $\sem{\vdash_\omega \dup_A^\emptyset\colon A\iso A\otimes A} = x \mapsto (x,x)$.\qed
\end{lemma}

Now, given an iso $\omega : A\iso B\otimes C$ and $\omega' : B \iso A \otimes C'$
where $C, C'$ represent garbage, we can build an iso from $A\iso B$ as follow
where the variables $x, y, z$ (and their indices) respectively correspond to the
first, second, and third wire of~\Cref{fig:garbage-removal}: 

\begin{definition}[Garbage Removal Iso]~\rm
  We defined $\garRem{\omega}{\omega'}$ by $\{x_1~\iso~
\letv{\pv{x_2}{y}}{\omega~x_1}{} 
             \letv{\pv{x_3}{z}}{\dup_B^\emptyset~x_2}{} 
            \letv{x_4}{\omega^{-1}~\pv{x_3}{y}}{}
            \letv{\pv{z_2}{y_2}}{\omega'~z}{}
             \letv{z_3}{(\dup_B^\emptyset)^{-1}~\pv{z_2}{x_4}}{} 
             \letv{z_4}{\omega'^{-1}~\pv{z_3}{y_2}}{}
             z_4\}$.
\end{definition}

\begin{lemma}[Garbage Removal is well-typed]
  \label{lem:garbage-removal-typed}
  Given $\omega : A\iso B\otimes C$ and $\omega' : B \iso A \otimes C'$ then
  $\garRem{\omega}{\omega'}$ is a well-typed iso of type $A\iso B$.\qed
\end{lemma}

\begin{lemma}[Garbage Removal Semantics]\label{lem:garb-remove-sem}
  Given $\omega : A\iso B\otimes C$ and $\omega' : B \iso A \otimes C'$ and any
  well-typed value $v$ of type $A$, such that if $\omega~v \to^* \pv{v_1}{v_2}$
  and $\omega'~v_1\to^* \pv{v_3}{v_4}$ then $v_3 = v$,  
  then if $\garRem{\omega}{\omega'}~v \to^* v_5$ then $v_1 = v_5$.
  The denotational semantics $\sem{\omega,\omega'\vdash_\omega \garRem{\omega}{\omega'}}(x)$ is
  $\sem\omega (x)$ if $(\sem{\omega'}((\sem\omega (x))_1))_1 = x$ and $\bot$ otherwise.\qed
	% \[
	% 	\sem{\omega,\omega'\vdash_\omega \garRem{\omega}{\omega'}} = x \mapsto
	% 	\left\{\begin{array}{ll}
	% 		\sem\omega (x) & \text{if $(\sem{\omega'}((\sem\omega (x))_1))_1 = x$,} \\
	% 		\bot & \text{else.}
	% 	\end{array}\right.
	% \]
\end{lemma}


\input{rtm2}









\subsection{Capturing every computable function}

\todo[inline]{A supprimer de ``garbageremoval.tex''}

With this encoding, every iso $\omega : A\iso B$ can be turned into another iso
$\floor{\omega} : [\opn{Enc}] \iso [\opn{Enc}]$ by composing $\floor{-}_A$,
followed by $\omega$, followed by $\floor{-}_B^{-1}$. This is in particular the
case for isos that are the images of a Turing Machine. We are now ready to see
how every computable function $f$ from $\interp{A} \to \interp{B}$ can be turned
into an iso whose semantics is $f$.
Given a computable function $f : \interp{A} \to \interp{B}$, call $M_f$ the
RTM computing $f$. Since $f$ is in $\PInj$, its output
uniquely determines its input. Following~\cite{bennett1973logical}, there exists
another Turing Machine $M_f'$ which, given the output of $M_f$ recovers the
initial input.
In our encoding of a RTM, the iso will have another additional garbage
which consist of a natural number, i.e. the number of steps of the RTM $M_f$.
Using $\garRem{\opn{isos}(M_f)}{\opn{isos}(M_f')}$ we can obtain a single iso,
from the encoding of $A$ to the encoding of $B$, without any garbage left.
This also ensures that $\sem{\garRem{\opn{isos}(M_f)}{\opn{isos}(M_f')}}(x)
= (\sem{\opn{isos}(M_f)}(x))_1$, for any input $x$.

\begin{theorem}[Computable function as Iso]
	\label{th:computable}
	Given a computable function $f\colon \interp{A} \to \interp{B}$, let $g\colon
	\interp{[\opn{Enc}] \otimes [\opn{Enc}]} \to \interp{[\opn{Enc}] \otimes
	[\opn{Enc}]}$ be defined as $g = \interp{\floor{-}_B} \circ f \circ
	\interp{\floor{-}_A^{-1}}$, and let $\omega\colon A \iso B$ be defined as $\{x~\iso~
	\letv{y}{\floor{x}_A}{} 
    \letv{y'}{\garRem{\opn{isos}(M_g)}{\opn{isos}(M_g')}~y}{}
    \letv{z}{\floor{y'}_B^{-1}}{z}\}$.
  Then $\interp{\omega} = f$.\qed
\end{theorem}

